Probing fragmentation and velocity sub-structure in the massive NGC 6334 filament with ALMA

Herschel surveys of Galactic clouds support a paradigm for low-mass star formation in which dense filaments play a crucial role. The detailed fragmentation properties of star-forming filaments remain poorly understood, however, and the validity of the filament paradigm in the high-mass regime is still unclear. To investigate the density/velocity structure of the filament in the high-mass star-forming region NGC6334, we conducted ALMA observations in the 3mm continuum and the N2H+(1-0) line at ~3arcsec resolution. The filament was detected in both tracers. We identified 26 cores at 3mm and 5 velocity-coherent fiber-like features in N2H+ within the filament. The typical length of, and velocity difference between, the fiber-like features of the NGC6334 filament are reminiscent of the properties for the fibers of the low-mass star-forming filament B211/B213. Only 2 or 3 of the 5 velocity-coherent features are well aligned with the filament and may represent genuine, fiber sub-structures. The core mass distribution has a peak at ~10Msun. They can be divided into 7 groups of cores, closely associated with ArTeMiS clumps. The projected separation between cores and the projected spacing between clumps are roughly consistent with the effective Jeans length in the filament and a physical scale of about 4 times the filament width, respectively, suggesting a bimodal filament fragmentation process. Despite being one order of magnitude denser and more massive than the B211/B213 filament, the NGC6334 filament has a similar density/velocity structure. The difference is that the cores in NGC6334 appear to be an order of magnitude denser and more massive than the cores in Taurus. This suggests that dense filaments may evolve and fragment in a similar manner in low- and high-mass star-forming regions, and that the filament paradigm may hold in the intermediate-mass (if not high-mass) star formation regime.

==> getsources_table.tex <==
%Threshold of separation between dust and N2H+ core is 3.0arcsec 
\begin{table*} 
%\tiny 
\centering 
\caption{Results of compact source extractions on the ALMA 3.1 mm continuum map \label{table:cont_getsources}} 
\scalebox{0.55}{
\begin{tabular}{lcccccccccccc} 
\hline 
ID$^{\dag}$ & RA & DEC & $R_{\rm major} \times R_{\rm minor}$ & PA      &  S$_{\rm 3.1mm}^{\rm peak} & S/N $  & $S_{\rm 3.1mm}^{\rm tot}$ & $M_{\rm tot}$ & $\overline{n_{\rm H_2}}$ & Velocity ranges at which source is detected in N$_2$H$^+$  & Association with N$_2$H$^+$ features \\ 
    & [h:m:s] & [d:m:s] & $^{*}$ & [deg] &   [mJy/beam] & [$\sigma$] & [mJy] & [$M_{\odot}$]$^{**}$  & [$\times$10$^6$ cm$^{-3}$]  & [km s$^{-1}$]  &  \\ 
\hline 
1        & 17:20:41.78 & -35:48:09.1 & 2.$\arcsec$9$\times$2.$\arcsec$3 (0.02 pc $\times$ 0.02 pc) &93  & 6.9$\pm$0.6 &34.3 & 13.5$\pm$0.6 & 13.8 & 5.1 &  & No N$_2$H$^+$ \\  
{\bf 2}  & 17:20:43.14 & -35:47:54.9 & 2.$\arcsec$6$\times$1.$\arcsec$6 (0.02 pc $\times$ 0.01 pc) &112 & 5.5$\pm$0.3 &27.3 & 12.3$\pm$0.3 & 33.9 & 24.1 & [-2.2,-1.8] & F-2 \\  
3        & 17:20:45.00 & -35:46:42.7 & 1.$\arcsec$2$\times$1.$\arcsec$2 (0.01 pc $\times$ 0.01 pc) &67  & 2.5$\pm$0.2 &12.3 & 2.8$\pm$0.3 & 7.7   & 28.1 & -1.2 & F-2(marginal)$^{\ddag}$ \\  
{\bf 4}  & 17:20:43.55 & -35:47:51.7 & 2.$\arcsec$2$\times$2.$\arcsec$2 (0.02 pc $\times$ 0.02 pc) &154 & 2.2$\pm$0.3 &10.8 & 3.8$\pm$0.3 & 10.6  & 6.1 & [-1.4,-1.2] & F-2 \\  
{\bf 5}  & 17:20:43.15 & -35:47:46.5 & 2.$\arcsec$7$\times$2.$\arcsec$1 (0.02 pc $\times$ 0.02 pc) &97  & 2.2$\pm$0.3 &10.7 & 4.0$\pm$0.3 & 11.1  & 5.0 & [-2.6,-2.4],[-2.0,-1.8] & F-1/F-2 \\  
{\bf 6}  & 17:20:44.65 & -35:46:54.3 & 2.$\arcsec$1$\times$2.$\arcsec$1 (0.02 pc $\times$ 0.02 pc) &97  & 1.6$\pm$0.3 &7.8 & 2.7$\pm$0.3 & 7.5    & 4.9 & [-3.0,-2.8],[-1.8,-1.2] & F-1/F-2 \\  
{\bf 7}  & 17:20:44.52 & -35:47:00.7 & 2.$\arcsec$6$\times$1.$\arcsec$7 (0.02 pc $\times$ 0.01 pc) &65  & 1.4$\pm$0.4 &7.1 & 2.3$\pm$0.4 & 6.3    & 4.2 & [-3.8,-2.8] & F-1 \\  
{\bf 8}  & 17:20:44.47 & -35:47:17.1 & 2.$\arcsec$6$\times$2.$\arcsec$4 (0.02 pc $\times$ 0.02 pc) &28  & 1.5$\pm$0.4 &7.6 & 2.9$\pm$0.4 & 8.0    & 3.0 & [-2.8, -2.6],[-1.8,-1.2] & F-1/F-2 \\  
{\bf 9}  & 17:20:40.42 & -35:48:51.2 & 2.$\arcsec$2$\times$2.$\arcsec$2 (0.02 pc $\times$ 0.02 pc) &21  & 2.0$\pm$0.4 &9.9 & 3.2$\pm$0.4 & 8.9    & 5.0 & [-2.6,-1.4] &  \\  
{\bf 10} & 17:20:41.25 & -35:48:18.4 & 3.$\arcsec$6$\times$2.$\arcsec$8 (0.03 pc $\times$ 0.02 pc) &1   & 2.3$\pm$0.5 &11.6 & 5.1$\pm$0.5 & 14.1  & 2.8 & [-3.6,-2.6] & F-1 \\  
11       & 17:20:39.05 & -35:49:20.8 & 2.$\arcsec$2$\times$2.$\arcsec$2 (0.02 pc $\times$ 0.02 pc) &129 & 1.7$\pm$0.5 &8.5 & 2.7$\pm$0.5 & 7.5    & 4.2 &  & No N$_2$H$^+$ \\  
{\bf 12} & 17:20:39.27 & -35:49:16.8 & 2.$\arcsec$1$\times$2.$\arcsec$1 (0.02 pc $\times$ 0.02 pc) &64  & 2.2$\pm$0.6 &10.8 & 3.4$\pm$0.6 & 9.2   & 6.1 & [-3.8,-3.0] &  \\  
{\bf 13} & 17:20:39.35 & -35:49:01.7 & 3.$\arcsec$8$\times$2.$\arcsec$6 (0.03 pc $\times$ 0.02 pc) &140 & 1.6$\pm$0.6 &7.9 & 3.4$\pm$0.6 & 9.4    & 1.9 & [-3.8,-1.8] &  \\  
{\bf 14} & 17:20:45.51 & -35:46:33.7 & 1.$\arcsec$9$\times$1.$\arcsec$9 (0.02 pc $\times$ 0.02 pc) &80  & 1.0$\pm$0.2 &5.1 & 1.6$\pm$0.2 & 4.4    & 3.8 & [-3.2,-2.8],[-2.2,-1.2] & F-1/F-2 \\  
15       & 17:20:40.97 & -35:48:21.4 & 4.$\arcsec$1$\times$2.$\arcsec$4 (0.03 pc $\times$ 0.02 pc) &83  & 2.0$\pm$0.5 &10.2 & 4.2$\pm$0.5 & 11.5  & 2.3 &  & No N$_2$H$^+$ \\  
{\bf 16} & 17:20:39.40 & -35:49:13.5 & 3.$\arcsec$5$\times$2.$\arcsec$7 (0.03 pc $\times$ 0.02 pc) &153 & 2.2$\pm$0.4 &10.8 & 4.8$\pm$0.4 & 13.3  & 2.8 & [-3.8,-2.6] &  \\  
17       & 17:20:41.58 & -35:48:37.5 & 3.$\arcsec$0$\times$2.$\arcsec$2 (0.02 pc $\times$ 0.02 pc) &64  & 2.4$\pm$0.6 &12.2 & 3.7$\pm$0.6 & 10.3  & 3.8 &  & No N$_2$H$^+$/Out of main filament \\  
18       & 17:20:43.36 & -35:48:47.0 & 4.$\arcsec$1$\times$2.$\arcsec$6 (0.03 pc $\times$ 0.02 pc) &67  & 3.4$\pm$0.8 &16.9 & 6.8$\pm$0.9 & 18.7  & 3.3 &  & No N$_2$H$^+$/Out of main filament \\  
19       & 17:20:42.35 & -35:48:34.3 & 3.$\arcsec$3$\times$2.$\arcsec$9 (0.03 pc $\times$ 0.02 pc) &61  & 3.0$\pm$1.3 &15.0 & 6.4$\pm$1.5 & 17.6  & 3.6 &  & No N$_2$H$^+$ \\  
{\bf 20} & 17:20:41.63 & -35:48:03.3 & 3.$\arcsec$9$\times$2.$\arcsec$7 (0.03 pc $\times$ 0.02 pc) &30  & 1.4$\pm$0.2 &7.0 & 3.0$\pm$0.3 & 8.4    & 1.6 & [-3.4,-2.4] & F-1 \\  
{\bf 21} & 17:20:43.68 & -35:47:48.4 & 3.$\arcsec$1$\times$2.$\arcsec$7 (0.03 pc $\times$ 0.02 pc) &46  & 1.3$\pm$0.3 &6.6 & 2.7$\pm$0.3 & 7.3    & 1.9 & [-2.2,-1.2] & F-2 \\  
{\bf 22} & 17:20:44.39 & -35:47:26.4 & 3.$\arcsec$7$\times$2.$\arcsec$5 (0.03 pc $\times$ 0.02 pc) &4   & 1.2$\pm$0.3 &5.9 & 2.5$\pm$0.3 & 6.8    & 1.5 & [-3.8,-3.2],[-1.8,-1.2] & F-1/F-2 \\  
{\bf 23} & 17:20:42.63 & -35:48:26.1 & 3.$\arcsec$2$\times$2.$\arcsec$6 (0.03 pc $\times$ 0.02 pc) &85  & 1.5$\pm$0.5 &7.3 & 2.3$\pm$0.6 & 6.4    & 1.7 & [-1.4,-1.2] &  \\  
24       & 17:20:41.88 & -35:49:01.8 & 3.$\arcsec$6$\times$2.$\arcsec$3 (0.03 pc $\times$ 0.02 pc) &53  & 1.4$\pm$0.4 &6.9 & 2.6$\pm$0.4 & 7.1    & 1.9 &  & No N$_2$H$^+$/Out of main filament \\  
\hline 
\end{tabular} 
}
\tablefoot{\tablefoottext{\dag}{IDs of 3.1 mm compact sources associated with N$_2$H$^+$ emission in two or more contiguous channels are labeled in bold.}\\
\tablefoottext{\ddag}{Marginal N$_2$H$^+$ detection since it is detected in only one channel for this source.}\\ 
\tablefoottext{$^*$}{Deconvolved FWHM source diameters along the major and minor axes.}\\ 
\tablefoottext{$^{**}$}{We adopted $T_{\rm dust}$ = 20 K for all sources, except for source ID 1 for which we assumed $T_{\rm dust}$ = 50 K (see Sect. \ref{sect:getsources}).} 
}
\end{table*} 

